Depth Anything 3: Recovering the Visual Space from Any Views

We present Depth Anything 3 (DA3), a model that predicts spatially consistent geometry from an arbitrary number of visual inputs, with or without known camera poses. In pursuit of minimal modeling, DA3 yields two key insights: a single plain transformer (e.g., vanilla DINO encoder) is sufficient as a backbone without architectural specialization, and a singular depth-ray prediction target obviates the need for complex multi-task learning. Through our teacher-student training paradigm, the model achieves a level of detail and generalization on par with Depth Anything 2 (DA2). We establish a new visual geometry benchmark covering camera pose estimation, any-view geometry and visual rendering. On this benchmark, DA3 sets a new state-of-the-art across all tasks, surpassing prior SOTA VGGT by an average of 44.3% in camera pose accuracy and 25.1% in geometric accuracy. Moreover, it outperforms DA2 in monocular depth estimation. All models are trained exclusively on public academic datasets.

==> figs/texs/teaser_small.tex <==
\begin{figure}[h]
    \vspace{0mm}
    \begin{center}
    \includegraphics[width=1\textwidth]{figs/pdfs/teaser_small.jpeg}
    \vspace{-5mm}
    \vspace{-2mm}
    \label{fig:teaser}
    \end{center}
\end{figure}

==> sections/0-abstract.tex <==
\begin{abstract}
We present Depth Anything 3 (DA3), a model that predicts spatially consistent geometry from an arbitrary number of visual inputs, with or without known camera poses. 
In pursuit of minimal modeling, DA3 yields two key insights:
a single plain transformer (\eg, vanilla DINO encoder) is sufficient as a backbone without architectural specialization, and a singular depth-ray prediction target obviates the need for complex multi-task learning. Through our teacher-student training paradigm, the model achieves a level of detail and generalization on par with Depth Anything 2 (\textit{DA2}).
We establish a new visual geometry benchmark covering camera pose estimation, any-view geometry and visual rendering. On this benchmark, DA3 sets a new state-of-the-art across all tasks, surpassing prior SOTA \textit{VGGT} by an average of 44.3\% in camera pose accuracy and 25.1\% in geometric accuracy. Moreover, it outperforms \textit{DA2} in monocular depth estimation. All models are trained exclusively on public academic datasets.
\end{abstract}

==> sections/metric.tex <==

\subsection{Metric}
\subsubsection{Metric Depth Estimation}
We train a metric depth estimation model. Following Metric3Dv2~[], we apply canonical camera space transformation to address depth ambiguity caused by varying focal lengths. Specifically, we rescale the ground-truth depth using ratio $f^c/f$, where $f^c$ and $f$ denote the canonical focal length and camera focal length, respectively. To ensure sharp details, we employ Depth-Anything-3-Teacher~(Section xx) model's prediction to supervise the training of metric depth model. We align the scale and shift of the teacher model's predicted depths with the ground-truth metric depth labels for supervision. We trained our metric depth model on 13 datasets, including Taskonomy~[], DIML (Outdoor)~[], DDAD~[], Argoverse~[], Lyft~[], Pandaset~[], Waymo~[], ScanNet++~[], ARKitScenes~[], Map-free~[], DSEC~[], Driving Stereo~[] and Cityscapes~[] datasets. For stereo datasets, we leverage the prediction of FoundationStereo~[] as training labels. The training objective is a weighted sum of depth loss $\mathcal{L}_{depth}$, $\mathcal{L}_{grad}$ and sky-mask loss $\mathcal{L}_{sky}$.

\noindent \textbf{Implementation details.} The training largely follows that of the monocular Depth-Anything-3-Teacher model. All images are trained at a base resolution of 504 with varying aspect ratios (1:1, 1:2, 16:9, 9:16, 3:4, 1:1.5, 1.5:1, 1:1.8). We employ AdamW optimizer and set the learning rate for encoder and decoder to 5e-6 and 5e-5, respectively. We apply random rotation augmentation where training images are rotated at 90 or 270 degree with 5\% probability. We set canonical focal length $f^c$ to 300. We use the aligned prediction from Depth-Aynthing-3-Teacher as supervision. With a probability of 20\%, we use the original ground-truth labels for training. We train with batch size of 64 for 160K iterations.

\input{tables/metric.tex}
\noindent \textbf{Results.}
We compare with the state-of-the-art metric depth estimation methods, including UniDepthV1~[], UniDepthV2~[], Metric3Dv2~[], DepthPro~[] and MoGe-2~[], on 5 benchmarks, \textit{i.e.}, NYU-D~[], KITTI, ETH3D, SUNRGBD and DIODE (indoor). As shown in Table~\ref{tab:metric}, our method outperforms other works on ETH3D while performing comparably on other benchmarks. 

\textbf{Ablation Study.} We also ablate the design for incorporating Depth-Anything-3-Teacher for supervision. As shown in Table~\ref{tab:metric}, removing Depth-Anything-3-Teacher does not quantitaively degrade the performance. However, as shown in Fig.~\ref{fig:metric-abl}, the sharpness is greatly improved, demonstrating the effectiveness of Depth-Anything-3-Teacher for improving the sharpness.

\begin{figure}
    \centering
    \includegraphics[width=\linewidth]{figs/pdfs/metric-abl.pdf}
    \caption{\textbf{Effectiveness of Depth-Anything-3-Teacher for supervising metric depth estimation.} Incorporating Depth-Anything-3-Teacher for supervision significantly improves the metric depth sharpness.}
    \label{fig:metric-abl}
\end{figure}

==> tables/ablation_app.tex <==
\begin{table}[tb]
    \caption{
        \textbf{More ablations for single transformer.} We evaluate the effects of the dual-DPT head, teacher label supervision, and the pose conditioning module. Methods marked with “*” are evaluated with ground-truth pose fusion.
    }
    \vspace{-2mm}
    \label{tab:abl_dav3_app}
    \begin{center}
    \resizebox{0.925\linewidth}{!}{
    \begin{tabular}{lcccccccccc}
        \toprule
        \multirow{2}{*}[-4pt]{\textbf{Methods}} 
        & \multicolumn{2}{c}{\textbf{ \picodataset }} 
        & \multicolumn{2}{c}{\textbf{ ETH3D }} 
        & \multicolumn{2}{c}{\textbf{ DTU }} 
        & \multicolumn{2}{c}{\textbf{ 7Scenes }} 
        & \multicolumn{2}{c}{\textbf{ ScanNet++ }} 
        \\
        \cmidrule(lr){2-3} \cmidrule(lr){4-5} \cmidrule(lr){6-7} \cmidrule(lr){8-9} \cmidrule(lr){10-11} 
        & Auc3$\uparrow$ & F1$\uparrow$ 
        & Auc3$\uparrow$ & F1$\uparrow$ 
        & Auc3$\uparrow$ & CD$\downarrow$ 
        & Auc3$\uparrow$ & F1$\uparrow$ 
        & Auc3$\uparrow$ & F1$\uparrow$  \\
        \midrule
        a. Full Model      
        & 39.2 & 47.0 
        & 21.0 & 55.4 
        & 45.8 & 3.82 
        & 26.2 & 47.6 
        & 30.3 & 51.1 \\
        \midrule
        d. w/o Dual DPT    
        & 5.59 & 11.5 
        & 13.6 & 33.4 
        & 21.7 & 5.14 
        & 14.2 & 49.4 
        & 26.5 & 46.6 \\
        e. w/o Teacher     
        & 11.2 & 16.0 
        & 16.2 & 57.6 
        & 52.5 & 3.29 
        & 23.3 & 40.3 
        & 26.2 & 47.7 \\
        \midrule
        f. w/o Pose Cond.*
        &  & 65.8
        &  & 63.2
        &  & 3.65
        &  & 58.4
        &  & 62.8 \\
        g. w/ Pose Cond.*
        &  & 73.8
        &  & 70.9
        &  & 2.14
        &  & 46.0
        &  & 65.7 \\
        \bottomrule
    \end{tabular}
    }
    \end{center}
\end{table}



==> tables/metric_ablation.tex <==
\begin{table}[tb]
    \centering
    \caption{\textbf{Ablation study.}}
    \resizebox{0.925\linewidth}{!}{
    \begin{tabular}{lcccccccccc}
        \toprule
        \multirow{2}{*}[-4pt]{\textbf{Methods}} 
        & \multicolumn{2}{c}{\textbf{ NYUv2 }} 
        & \multicolumn{2}{c}{\textbf{ KITTI }} 
        & \multicolumn{2}{c}{\textbf{ ETH3D }} 
        & \multicolumn{2}{c}{\textbf{ SUN-RGBD }} 
        & \multicolumn{2}{c}{\textbf{ DIODE }} 
        \\
        \cmidrule(lr){2-3} \cmidrule(lr){4-5} \cmidrule(lr){6-7} \cmidrule(lr){8-9} \cmidrule(lr){10-11} 
        & $\delta_1$$\uparrow$ & AbsRel$\downarrow$ 
        & $\delta_1$$\uparrow$ & AbsRel$\downarrow$ 
        & $\delta_1$$\uparrow$ & AbsRel$\downarrow$ 
        & $\delta_1$$\uparrow$ & AbsRel$\downarrow$ 
        & $\delta_1$$\uparrow$ & AbsRel$\downarrow$  \\
        \midrule
        w/ teacher & 0.966 & 0.073 & 0.947 & 0.086 & 0.906 & 0.105 & 0.973 & 0.104 & 0.824 & 0.132 \\
        w/o teacher & 0.969 & 0.066 & 0.965 & 0.067 & 0.907 & 0.105 & 0.975 & 0.099 & 0.816 & 0.134 \\
        \bottomrule
    \end{tabular}
    }
    \label{tab::metric_ablation}
\end{table}
